PCPATCH: software for the topological construction of multigrid relaxation methods

Effective relaxation methods are necessary for good multigrid convergence. For many equations, standard Jacobi and Gau{\ss}-Seidel are inadequate, and more sophisticated space decompositions are required; examples include problems with semidefinite terms or saddle point structure. In this paper we present a unifying software abstraction, PCPATCH, for the topological construction of space decompositions for multigrid relaxation methods. Space decompositions are specified by collecting topological entities in a mesh (such as all vertices or faces) and applying a construction rule (such as taking all degrees of freedom in the cells around each entity). The software is implemented in PETSc and facilitates the elegant expression of a wide range of schemes merely by varying solver options at runtime. In turn, this allows for the very rapid development of fast solvers for difficult problems.

==> code/Makefile <==
all: allen-cahn/table-allen-cahn.tex elasticity/table-elasticity.tex \
	hdivcurl/table-Hdiv-dim0.tex hdivcurl/table-Hdiv-dim1.tex \
	hdivcurl/table-Hcurl-dim0.tex \
	stokes/table-stokes.tex

allen-cahn/table-allen-cahn.tex allen-cahn/table-allen-cahn.json: allen-cahn/allen-cahn.py
	(cd allen-cahn; mpiexec -n 28 python allen-cahn.py; cd ../)

elasticity/table-elasticity.tex elasticity/table-elasticity.json: elasticity/elasticity.py
	(cd elasticity; mpiexec -n 28 python elasticity.py; cd ../)

hdivcurl/table-Hdiv-dim0.tex hdivcurl/table-Hdiv-dim0.json: hdivcurl/hdivcurl.py
	(cd hdivcurl; mpiexec -n 28 python hdivcurl.py --op div --construct-dim 0; cd ../)

hdivcurl/table-Hdiv-dim1.tex hdivcurl/table-Hdiv-dim1.json: hdivcurl/hdivcurl.py
	(cd hdivcurl; mpiexec -n 28 python hdivcurl.py --op div --construct-dim 1; cd ../)

hdivcurl/table-Hcurl-dim0.tex hdivcurl/table-Hcurl-dim0.json: hdivcurl/hdivcurl.py
	(cd hdivcurl; mpiexec -n 28 python hdivcurl.py --op curl --construct-dim 0; cd ../)

stokes/table-stokes.tex stokes/table-stokes.json: stokes/stokes.py
	(cd stokes; mpiexec -n 28 python stokes.py; cd ../)


==> code/hdivcurl/table-Hdiv-dim1.tex <==
\begin{tabular}{cc|ccccc}
\toprule
\# refinements & \# degrees of freedom & \multicolumn{5}{c}{$\alpha$} \\
 && $10^0$ & $10^1$ & $10^2$ & $10^3$ & $10^4$ \\
\midrule
1 & $1.26 \times 10^{4}$ & 40 & 42 & 43 & 44 & 44\\
2 & $9.84 \times 10^{4}$ & 42 & 43 & 43 & 43 & 43\\
3 & $7.78 \times 10^{5}$ & 45 & 45 & 45 & 45 & 45\\
4 & $6.18 \times 10^{6}$ & 46 & 47 & 47 & 47 & 47\\
\bottomrule
\end{tabular}

